Multilingual LLMs are Better Cross-lingual In-context Learners with Alignment

In-context learning (ICL) unfolds as large language models become capable of inferring test labels conditioned on a few labeled samples without any gradient update. ICL-enabled large language models provide a promising step forward toward bypassing recurrent annotation costs in a low-resource setting. Yet, only a handful of past studies have explored ICL in a cross-lingual setting, in which the need for transferring label-knowledge from a high-resource language to a low-resource one is immensely crucial. To bridge the gap, we provide the first in-depth analysis of ICL for cross-lingual text classification. We find that the prevalent mode of selecting random input-label pairs to construct the prompt-context is severely limited in the case of cross-lingual ICL, primarily due to the lack of alignment in the input as well as the output spaces. To mitigate this, we propose a novel prompt construction strategy -- Cross-lingual In-context Source-Target Alignment (X-InSTA). With an injected coherence in the semantics of the input examples and a task-based alignment across the source and target languages, X-InSTA is able to outperform random prompt selection by a large margin across three different tasks using 44 different cross-lingual pairs.

==> rebuttal.tex <==

% The major concerns per the reviewer is as follows:-

% On average we scored 3.5 in soundness (3rd has given us a 2 else all are 4) and 3.5 in excitement (1st has given us 2.5 else all =<3.5)

% Reviewer one:-
% He has scored the lowest in excitement out of all 4 reviews (Score of 2.5, others have scored 3.5)
%     1. Not generalizable to another task, will require writing the prompt.
%     2. the similarity retrieval part is not novel.

% Reviewer two:-
% He generally is interested in our method and his rebuttals are more like questions on why we did it this way.
%     1. a couple of language pairs show detrimental performance (like English to German in CLS)
%     2. automatically doing task alignment leads to poorer performance 
%     3. Is it possible to use the same model for calculating sentence embeddings and classification (XGLM in this case)?
%     4. Were there any other alignment techniques that were considered but didn't make it to the final paper?

% Review three:-
% He has scored the lowest in Soundness out of all 4 reviews (Score of 2, others have scored 4)
%     1. Only classification tasks no generation tasks.
%     2. Some low-resource languages should also have been added to the mix
%     3. Experiments are done with a single 7B model.

% REBUTTLES

% related to only classification tasks.

%     IN THE FOLLOWING EN WAS SET AS src language.
    
%     XCOPA results (a commonsense QnA task):- no-examples, random-prompting, (0.559,0.561) (f1, the score is near random 0.5) Changing prompt don't lead to better results, i.e. current models are bad at cross-lingual commonsense reasoning.

%     Tydi (Open QA):- no-examples, random-prompting (0.06,0.03) (acc). Current models are not good language base or models are not good with QA tasks, and cross lingual reduces performance even further.

%     MQA (Read comprehension QA):- no-examples, random-prompting (0.238,0.214) (acc). No improvement,  i.e. current models are bad at cross-lingual reasoning for QA task?
    
%     While Larger LLMs have such reasoning capacity \cite{}, there is no multilingual model that we know of (Tho BLOOM 175B exists so be cautious here) which has better reasoning capacity. 
    
%     xglm 7.5B is the largest model in that series So we can it. Taking the fact that ICL improves with size as a fact
%                                                     or
%     Model scalability improves performance and is a well-known phenomenon (Cite glam, bloom, others). Hence we didn't decide to explore it, instead, we took the best possible model that can fit our hardware and came up with a model-agnostic model.

%                                                     or

%     as shown by text generation results we need better multilingual autoregressive models for QA, commonsense reasoning. these models will only come if there more research interest the community towards Cross-Lingual/multilingual ICL

%     Only recently Alpaca model (~6B in size) has shown to be well reasonable because their training dataset is selected. There is no existing multilingual model of small size that has specifically been designed to be good at reasoning like alpaca. multilingual LLMs generally rely on web-scaped datasets to train upon and are rarely very big in size. This lack of reasoning of multilingual-LLMs is here to stay till a high quality model is created.

%     citations:-
%     ICL is a scales with model size (paper:- Language Models are Few-Shot Learners)
%     XGlm paper, Bloom paper model size scaling (paper:- Few-shot Learning with Multilingual Language Models, BLOOM: A 176B-Parameter Open-Access Multilingual Language Model)

    

% Results on xglm-1.7B and bloom-7b1

% xglm-1.7B on MARC

% src,tar,f1
% en,de,0.555
% en,es,0.422
% en,fr,0.743
% en,ja,0.604
% en,zh,0.784

% xglm-1.7B on CLS

% src,tar,f1
% en,de,0.711
% en,fr,0.382
% en,jp,0.395

% xglm-1.7B on Hateval

% src,tar,f1
% en,es,0.370

% bloom-7b1 on MARC

% src,tar,f1
% en,de,0.333
% en,es,0.613
% en,fr,0.490
% en,ja,0.573
% en,zh,0.333

% bloom-7b1 on CLS

% src,tar,f1
% en,de,0.333
% en,fr,0.355
% en,jp,0.508

% bloom-7b1 on Hateval

% src,tar,f1
% en,es,0.373

\begin{table*}[h]
\small
\centering
\adjustbox{max width=1.2\linewidth}{
\begin{tabular}{l|ccc|c}
 \hline
 \multirow{2}{*}{\backslashbox{ Setup}{ Target}} &\multicolumn{3}{c|}{CLS}&\multicolumn{1}{c}{HatEval}\\ 
 de&fr&ja&es
 \\
 \hline
{xglm-1.7B}&0.711&0.382&0.395&0.370\\
{xglam-7.5B}&0.682&0.412&0.609&0.435\\
{ bloom-7.1B}&0.0.33&0.355&0.508&0.0.373\\
\hline
\end{tabular}
}
\caption{Comparing the performance of different variants of multilingual generative models. We use English as the source language in all the experiments.}

\label{tab:auto-logic}
\end{table*}
\newpage
\section{Response to reviewers}
\subsection{General response}
We thank the anonymous reviewers greatly for their critical suggestions and appreciation of our work.

\subsection{Response to \#1}

[Lack of generalizability] We have already mentioned in the Limitations section (line no. 542-549) the challenges of designing these task aligners. To the best of our knowledge, this is the first attempt to explore the effects of task-based alignment for in-context learning, both in monolingual as well as cross-lingual settings. Automated aligners are definitely the best possible future work that can be derived from this paper. As [1] suggests, even powerful models like GPT-3 fall poorly in the case of cross-lingual tasks. We hope that our work will shed light on the direction to address the same.

[Missing references] Thank you for bringing this to our attention. We will definitely add discussions on the methods that retrieve similar examples from the training set during inference.
%from other areas regarding cross-lingual problems.

\subsection{Response to \#2}

[Language pairs with detrimental performance] Indeed we observed that for English-German task in the CLS dataset did not show performance improvement. In the case of English-Mandarin, we observe a performance drop with task aligners. As we analyzed in Section 3.1, the first case shows the inability of the underlying LLM to perform ICL in case of En-De pairs. As Wei et. al. [2] suggests, the pretraining prior plays a dominant role in the case of smaller models doing ICL. In the original paper [1] as well, XGLM-7B shows a high variation in performance across different language pairs. Added to this, in the second scenario (performance drop in Mandarin), the interplay between the pretraining distribution of the LLM and the task aligners is probably responsible for the deterioration. We hope that this opens a new door for possible future research.

[Static nature of task alignment] We have already mentioned in the Limitations section (line no. 542-549) the challenges of designing these task aligners. To the best of our knowledge, this is the first attempt to explore the effects of task-based alignment for in-context learning, both in monolingual as well as cross-lingual settings. Automated aligners are definitely the best possible future work that can be derived from this paper. As [1] suggests, even powerful models like GPT-3 fall poorly in the case of cross-lingual tasks. We hope that our work will shed light on the direction to solve the same.

[Question regarding semantic alignment] This is indeed a very interesting take on the semantic alignment part. The only caveat is since autoregressive LLMs like XGLM usually do not support bidirectional context like BERT, getting a fixed length representation of the input examples is tricky (since a fixed position CLS token like BERT will not accumulate the representations of the subsequent tokens via causal attention). One may seek to use another pass of prompting strategy beforehand to select similar examples, but the computational cost incurred will be much higher than using small models like Sentence-BERT. But indeed, this can be a promising research direction to explore.

Question regarding task alignment: The primary hypothesis behind task alignment was to transfer task-specific signals from the source language to the target. While translating a few examples might help this transfer, there are a few intuitive challenges: 1) the prompt context will become twice as long without providing any additional information (the model still needs to generalize only from the examples given), 2) a bottleneck posed by the translation quality, 3) if one simply uses translated examples only, the chances of generalization from a high resource language is lowered.

Question regarding other alignment methods: We indeed experimented with two other alignment methods: 1) selecting examples with diversity (non-similar examples in the source context), and, 2) mixing examples from a third language that is similar to the target (e.g., Japanese when the target is Mandarin, etc.). However, in the first case, we observed performance deterioration compared to random example selection. In the second case, there was no improvement compared to semantic alignment.

Suggestion on Figure 1: Thanks a lot for bringing this to our attention. We will include a clearer description in the camera-ready version.

\subsection{Response to \#3} 

Only classification tasks: We experimented with question-answering and machine reading comprehension while designing our research. With open-domain QA using the Tydi dataset, the base LLM provided near-random performance; in fact, performance dropped with 8-shot random prompting (0.03 accuracy) compared to zero-shot (0.06 accuracy). Similar behavior was observed in the case of the MQA (reading comprehension) dataset (accuracy dropped from 0.238 to 0.214 from zero-shot to random-prompts). Language models with fewer parameters tend to have very weak reasoning capabilities in an ICL setting. XGLM-7.5B is the largest, open-sourced multilingual LLM that we could work on (next in scale is Bloom-176B). This capped our extent of experimentation.

Variation with model scales and tuning: Thank you for your suggestion. As mentioned earlier, XGLM-7.5B is the largest multilingual LLM that we could use. We indeed experimented with smaller models like XGLM-1.7B and Bloom-7B. With both of them, the baseline performance using randomly selected prompts was much lower compared to XGLM-7.5B. We will include these results in the camera-ready version.

\subsection{Response to \#4} 

Thank you for appreciating our work. We will definitely include a clear definition of the task and semantic alignment in the camera-ready version.



==> results.tex <==


%\input{results.tex}

%\begin{table*}[ht]
%\centering
%\begin{tabular}{c|cccccc}
% \hline
% {\bf Source Language}&de&en&es&fr&ja&zh
% \\
% \hline
% de&$-$&$0.6$&$0.552$&$0.679$&$0.559$&$0.483$\\
% en &$0.4582$&$-$&$0.783$&$0.762$&$0.608$&$0.450$\\
% es&$0.377$&$0.771$&$-$&$0.740$&$0.643$&$0.568$\\
% fr&$0.376$&$0.752$&$0.879$&$-$&$0.565$&$0.589$\\
% ja&$0.333$&$0.754$&$0.733$&$0.0.690$&$-$&$0.697$\\
% zh&$0.333$&$0.682$&$0.839$&$0.536$&$0.675$&$-$\\
% \hline
% AVG&$0.375$&$0.713$&$0.757$&$0.681$&$0.610$&$0.557$\\
 
%\end{tabular}
%\caption{F1 Macro for AMCR using similarity}
%\end{table*}

%\begin{table*}[ht]
%\centering
%\begin{tabular}{c|cccccc}
% \hline
% {\bf Source Language}&de&en&es&fr&ja&zh
% \\
% \hline
% de&$-$&$0.567$&$0.701$&$0.768$&$0.645$&$0.333$\\
% en &$0.35582$&$-$&$0.888$&$0.826$&$0.727$&$0.333$\\
% es&$0.334$&$0.784$&$-$&$0.806$&$0.779$&$0.333$\\
% fr&$0.336$&$0.783$&$0.827$&$-$&$0.766$&$0.333$\\
% ja&$0.333$&$0.796$&$0.864$&$0.0.847$&$-$&$0.345$\\
% zh&$0.333$&$0.682$&$0.872$&$0.543$&$0.734$&$-$\\
% \hline
% AVG&$0.338$&$0.722$&$0.830$&$0.758$&$0.730$&$0.335$\\
% 
%\end{tabular}
%\caption{F1 Macro for AMCR using logic}
%\end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cccccc}
%  \hline
%  {\bf Source Language}&de&en&es&fr&ja&zh
%  \\
%  \hline
%  de&$-$&$0.721$&$0.756$&$0.847$&$0.760$&$0.333$\\
%  en &$0.382$&$-$&$0.891$&$0.858$&$0.783$&$0.335$\\
%  es&$0.348$&$0.857$&$-$&$0.875$&$0.851$&$0.334$\\
%  fr&$0.356$&$0.849$&$0.906$&$-$&$0.825$&$0.336$\\
%  ja&$0.333$&$0.832$&$0.890$&$0.0.845$&$-$&$0.348$\\
%  zh&$0.333$&$0.717$&$0.883$&$0.684$&$0.809$&$-$\\
%  \hline
%  AVG&$0.350$&$0.795$&$0.865$&$0.822$&$0.805$&$0.337$\\
 
% \end{tabular}
% \caption{F1 Macro for AMCR using logic and similarity}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cccc}
%  \hline
%  {\bf Source Language}&de&en&fr&ja
%  \\
%  \hline
%  de&$-$&$0.502$&$0.643$&$0.657$\\
%  en &$0.677$&$-$&$0.505$&$0.691$\\
%  fr&$0.572$&$0.746$&$-$&$0.743$\\
%  ja&$0.344$&$0.617$&$0.481$&$-$\\
%  \hline
%  AVG&$0.531$&$0.621$&$0.543$&$0.697$\\
 
% \end{tabular}
% \caption{F1 Macro for CLS using Similar}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cccc}
%  \hline
%  {\bf Source Language}&de&en&fr&ja
%  \\
%  \hline
%  de&$-$&$0.618$&$0.741$&$0.753$\\
%  en &$0.620$&$-$&$0.696$&$0.752$\\
%  fr&$0.511$&$0.782$&$-$&$0.840$\\
%  ja&$0.339$&$0.658$&$0.697$&$-$\\
%  \hline
%  AVG&$0.490$&$0.686$&$0.711$&$0.782$\\
% \end{tabular}
% \caption{F1 Macro for CLS using Logic}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cccc}
%  \hline
%  {\bf Source Language}&de&en&fr&ja
%  \\
%  \hline
%  de&$-$&$0.622$&$0.788$&$0.779$\\
%  en &$0.588$&$-$&$0.778$&$0.794$\\
%  fr&$0.524$&$0.821$&$-$&$0.834$\\
%  ja&$0.339$&$0.701$&$0.705$&$-$\\
%  \hline
%  AVG&$0.483$&$0.715$&$0.757$&$0.803$\\
 
% \end{tabular}
% \caption{F1 Macro for CLS using Logic and similarity}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cc}
%  \hline
%  {\bf Source Language}&es&en \\
%  \hline
%  es&$-$&$0.284$\\
%  en&$0.493$&$-$\\
%  \hline
%  AVG&$0.493$&$0.284$\\
 
% \end{tabular}
% \caption{F1 Macro for Hateval using Similar}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cc}
%  \hline
%  {\bf Source Language}&es&en \\
%  \hline
%  es&$-$&$0.269$\\
%  en&$0.499$&$-$\\
%  \hline
%  AVG&$0.499$&$0.269$\\
 
% \end{tabular}
% \caption{F1 Macro for Hateval using Logic}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{c|cc}
%  \hline
%  {\bf Source Language}&es&en \\
%  \hline
%  es&$-$&$0.269$\\
%  en&$0.542$&$-$\\
%  \hline
%  AVG&$0.542$&$0.269$\\
 
% \end{tabular}
% \caption{F1 Macro for Hateval using Logic and similar}
% \end{table*}
